Serre's constant of elliptic curves over the rationals

Let $E$ be an elliptic curve without complex multiplication defined over the rationals. The purpose of this article is to define a positive integer $A(E)$, that we call the {\it Serre's constant associated to $E$}, that gives necessary conditions to conclude that $\rho_{E,m}$, the mod m Galois representation associated to $E$, is non-surjective. In particular, if there exists a prime factor $p$ of $m$ satisfying ${\rm val}_p(m) > {\rm val}_p(A(E))>0$ then $\rho_{E,m}$ is non-surjective. {Conditionally under Serre's Uniformity Conjecture, w}e determine all the Serre's constants of elliptic curves without complex multiplication over the rationals that occur infinitely often. Moreover, we give all the possible combination of mod $p$ Galois representations that occur for infinitely many non-isomorphic classes of non-CM elliptic curves over $\mathbb{Q}$, and the known cases that appear only finitely. We obtain similar results for the possible combination of maximal non-surjective subgroups of ${\rm GL}_2(\mathbb{Z}_p)$. Finally, we conjecture all the possibilities of these combinations and in particular all the possibilities of these Serre's constant.

==> table_g3max_remain_RP.tex <==
 {
 \tiny
%\begin{table}[h]
\begin{center}
\begin{tabular}{cc}
\begin{tabular}{|c|c|c|}
\hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=3$}\\
\hline
 \rowcolor{white}   \texttt{[2B,7Ns]} & $(-16,2)$ & $2^4 3^3 5^3$ \\ 
& $(-1,0),(-1,-1)$ & 0 \\ 
 \hline
\texttt{[2Cn,7Nn]} & $(0,3)$ & $2^6 3^3$ \\ 
 \hline
\texttt{[2Cn,7Ns]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[3Nn,7Ns]} & $(0,-1),(0, 0)$ & 0 \\ 
& $(-96,1)$ & $-2^{15} 3^3$ \\ 
 \hline
\texttt{[3Ns,5Nn]} & $( 3, -1/2),(-1, -1/2)$ & 0 \\ 
& $(3, -1),(-1, -1)$ & \\ 
 \hline
   \hline
 \texttt{[4X3,7Nn]} & $(0, 3)$ & $2^6 3^3$ \\ 
 \hline
\texttt{[4X3,7Ns]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[4X7,13B]} & $\emptyset$ & $-$ \\ 
  \hline
  \texttt{[8X4,7Nn]} & $( 3, 0)$ & $2^6 3^3$ \\ 
 \hline
 \texttt{[8X4,7Ns]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[8X5,7Nn]} & $( -1, \pm 378)$ & $2^3 3^3 11^3$ \\ 
& $(3, 0)$ & $2^6 3^3$ \\ 
 \hline
\texttt{[8X5,7Ns]} & $( 5/2, \pm1431/16)$ & $3^3 5\, 7^5/2^7$\\ 
 \hline
 \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=4$}\\
\hline
 \rowcolor{white}  \hline
\texttt{[3Nn,5Cs]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[3Nn,5Ns.2.1]} & $( 0, 0)$ & 0 \\ 
 \hline
\texttt{[5S4,13B]} & $\emptyset$ & $-$ \\ 
  \hline
  \hline
\texttt{[2B,9XE]} & $( -1, \pm 1)$ & 0 \\ 
 \hline
\texttt{[4X7,7Nn]} & $( 8, 1)$ & $-2^{15}$ \\ 
& (-6, 3) & $2^6 3^3$ \\ 
& $(0, 0),(-8, 0)$ & 0 \\ 
& (-16008, -3/5) & $-2^{18} 3^3 5^3 23^3 29^3$ \\ 
& (120, 5) & $-2^{18} 3^3 5^3$ \\ 
& (-440, 2) & $-2^{15} 3^3 5^3 11^3$ \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=5$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[3B,7Nn]} & $( -1, 0), (-9, 0)$ & 0 \\ 
 \hline
\texttt{[5Nn,7B]} & $( -2, 7)$ & $3^3 5^3 17^3$ \\ 
& (0, -7) & $-3^3 5^3$ \\ 
 \hline
\hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=6$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[3B,7Ns]} & $( 1, 2)$ & $2^4 3^3 5^3$ \\ 
& (-1/9, 3) & $-2^{15} 3\,5^3$ \\ 
& $(-1, 0), (-9, -1)$ & 0 \\ 
&$ (-9, 0) (-1, -1)$ & \\ 
 \hline
\texttt{[3Ns,7Nn]} & $( -9, 1),(1/3, 1)$ & $-2^{15}$ \\ 
& $(-1, 0),(3, 0)$ & 0 \\ 
\hline
\texttt{[5B,7Nn]} & $\emptyset$ & $-$ \\ 
 \hline \hline
\texttt{[4X7,7Ns]} & $( 40, 3)$ & $-2^{15} 3\,5^3$ \\ 
& $(-24, 1)$ & $-2^{15} 3^3$ \\ 
& $(0, -1),(0, 0)$ & 0 \\ 
& $(-8, 0), (-8, -1)$ &  \\ 
 \hline
  \texttt{[4X7,9XE]} & $(-2195, -3/2)$ & $-2^2 3^7 5^3 439^3$ \\
\rowcolor{white}  & $( 0, \pm 1), (-8, \pm 1)$ & 0 \\ \hline
\hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=7$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[2Cn,11Nn]} & $( 2, 0)$ & $2^6 3^3$ \\ 
 \hline
\texttt{[3Nn,11Nn]} & $( 4, 66)$ & $2^3 3^3 11^3$ \\ 
& $(5/4, 0)$ & 0 \\ 
& $(2, 12)$ & $2^6 3^3$ \\ 
\hline
\texttt{[5S4,7Nn]} & $( 3, 3)$ & $2^6 3^3$ \\ 
& $(11, -1)$ & $2^3 3^3 11^3$ \\ 
& $(0, 0)$ & 0 \\ 
& $(-8, 1)$ & $-2^{15}$ \\  \hline \hline
\texttt{[4X3,11Nn]} & $( 2, 0)$ & $2^6 3^3$ \\ 
\hline
\texttt{[8X4,11Nn]} & $( 2, 0)$ & $2^6 3^3$ \\ 
 \hline
\texttt{[8X5,11Nn]} & $( 2, 0)$ & $2^6 3^3$ \\
 \hline 
 \end{tabular}
 &
 \begin{tabular}{|c|c|c|}
 \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=8$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[2B,11Nn]} & $( 2, 1/2),(2,-4)$ & $2^6 3^3$ \\ 
& $(4, 32)$ & $2^3 3^3 11^3$ \\ 
& $(5/4, -1)$ & 0 \\ 
 \hline
\texttt{[9XE,5S4]} & $( 0, \pm 1)$ & 0 \\ 
 \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=9$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[5B,7Ns]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[5Nn,13B]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[5S4,7Ns]} & $( -16, 1)$ & $-2^{15} 3^3$ \\ 
& $(0, -1),(0, 0)$ & 0 \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=10$}\\
\hline
 \rowcolor{white}  \hline
\texttt{[9XE,5B]} & $\emptyset$ & $-$ \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=13$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[5Nn,7Nn]} & $( 3/5, 2)$ & $-2^{15} 3^3 5^3 11^3$ \\ 
& $(-21/13, -3/5)$ & $-2^{18} 3^3 5^3 23^3 29^3$ \\ 
& $(-3/2, 5)$ & $-2^{18} 3^3 5^3$ \\ 
& $(-1, 0),(-1/2, 0)$ & 0 \\ 
 \hline \hline
 \texttt{[4X7,11Nn]} & $( 2, 40)$ & $-2^{15} 3\,5^3$ \\ 
& $(2, -6)$ & $2^6 3^3$ \\ 
& $(5/4, 0),(5/4, -8)$ & 0 \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=14$}\\
\hline
 \rowcolor{white}  \hline
\texttt{[3B,11Nn]} & $(2, -1/9)$ & $-2^{15} 3\,5^3$ \\
& $( 5/4, -1), (5/4, -9)$ & 0 \\ 
 \hline \hline
 \texttt{[9XE,7B]} & $\emptyset$ & $-$ \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=18$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[5Nn,7Ns]} & $(1, 2)$ & $2^4 3^3 5^3$ \\ 
& $(1/2, 3)$ & $-2^{15} 3\,5^3$ \\ 
& $( -1, -1),(-1/2, -1)$ & 0 \\ 
& $(-1/2, 0),(-1, 0)$ & \\ 
 \hline \hline
 \texttt{[9XE,5Nn]} & $( -1/2, \pm 1), (-1, \pm 1)$ & 0 \\ 
 \hline
  \hline
\rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=19$}\\
\hline
 \rowcolor{white}  \hline
\texttt{[5S4,11Nn]} & $( 4, 11)$ & $2^3 3^3 11^3$ \\ 
& $(5/4, 0)$ & 0 \\ 
& $(2, 3)$ & $2^6 3^3$ \\ 
 \hline \hline
 \rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=20$}\\
\hline
 \rowcolor{white} 
 \hline
\texttt{[5B,11Nn]} & $\emptyset$ & $-$ \\ 
 \hline
\texttt{[7Nn,13B]} & $\emptyset$ & $-$ \\ 
 \hline
  \hline
  \rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=26$}\\
\hline
 \rowcolor{white}  \hline 
\texttt{[9XE,13B]} & $\emptyset$ & $-$ \\ 
 \hline
  \hline  
 \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=27$}\\
 \rowcolor{white} \hline  
\texttt{[7Ns,13B]} & $\emptyset$ & $-$ \\ 
\hline
 \hline
 \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=32$}\\
 \hline   \rowcolor{white}
\texttt{[7B,11Nn]} & $\emptyset$ & $-$ \\ 
  \hline \hline
 \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=38$}\\
 \hline   \rowcolor{white}
\texttt{[5Nn,11Nn]} & $\emptyset$ & $-$ \\ 
 \hline \hline
  \rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=40$}\\
\hline
 \rowcolor{white} 
 \texttt{[9XE,7Nn]} & $( 0,\pm 1)$ & 0 \\ 
 \hline
 \hline
  \rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=54$}\\
\hline
 \rowcolor{white} \texttt{[9XE,7Ns]} & $(0,\pm 1),(-1,\pm 1)$ & 0 \\ 
  \hline
   \hline
  \rowcolor{light-gray} \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=56$}\\
 \hline     \rowcolor{white}
\texttt{[11Nn,13B]}& $\emptyset$ & $-$ \\ 
\hline
\hline
 \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=81$}\\
\hline   \rowcolor{white}
 \texttt{[7Nn,11Nn]}& $\emptyset$ & $-$ \\ 
\hline
\hline
 \rowcolor{light-gray}  \multicolumn{3}{|c|}{$g=111$}\\
\hline  
  \rowcolor{white}  \texttt{[9XE,11Nn]}& $\emptyset$ & $-$ \\
\hline
\hline
 \rowcolor{light-gray} \multicolumn{3}{|c|}{$g=112$}\\
 \hline   \rowcolor{white}
\texttt{[7Ns,11Nn]}& $\emptyset$ & $-$ \\ 
\hline
 \end{tabular}
 \end{tabular}
\captionof{table}{Remaining maximal modular curves of genus > 2}\label{rema}
 \end{center}
% \caption{Remaining Maximal curves}
 %\end{table}
 }
%Minimal quadratic twist with $j$-invariant $j_E=-2^2 3^7 5^3 439^3$ is $E:y^2 = x^3 - 1126035x + 459913278$. It has conductor $701784$.

\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline 
Type & Example & $j$-invariant & $\mathcal{N}_{\Q}(E)$  \\
\hline
\texttt{[4X7,9XE]}%\footnote{The modular curve associated to \texttt{[4X7,9XE]} has genus $6$ and we have found only one non-CM j-invariant, $j_E=-2^2 3^7 5^3 439^3$, the elliptic curve at  the table is the minimal quadratic twist.} 
& $-2^2 3^7 5^3 439^3$ & $y^2 = x^3 - 1126035x + 459913278$ & 701784\\
\hline
 \multirow{2}{*}{\texttt{13S4}} & \footnotesize$-\frac{2^{12}\cdot 5^3\cdot 11\cdot 13^4}{3^{13}}$&  \scriptsize $y^2 + y = x^3 + x^2 - 7653878762768x + 8080142566037338385$ & \scriptsize  374369283576145574257827 \\
\cline{2-4}
&  \footnotesize $\frac{2^{18}\cdot3^3\cdot 13^4\cdot 127^3\cdot 139^3\cdot 157^3\cdot 283^3\cdot 929}{5^{13}\cdot 61^{13}}$ & \scriptsize $y^2 + y = x^3 - 53690013976669148x + 4788368560731534924873003$ & \scriptsize 528531611786945 \\
\hline
\end{tabular}
\captionof{table}{Examples out of LMFDB: Genus $X_G >1$}\label{adicex}
\end{center}
